Probabilistic Forecasting of Real-Time Electricity Market Signals via Interpretable Generative AI

This paper introduces a generative AI approach to probabilistic forecasting of real-time electricity market signals, including locational marginal prices, interregional price spreads, and demand-supply imbalances. We present WIAE-GPF, a Weak Innovation AutoEncoder-based Generative Probabilistic Forecasting architecture that generates future samples of multivariate time series. Unlike traditional black-box models, WIAE-GPF offers interpretability through the Wiener-Kallianpur innovation representation for nonparametric time series, making it a nonparametric generalization of the Wiener/Kalman filter-based forecasting. A novel learning algorithm with structural convergence guarantees is proposed, ensuring that, under ideal training conditions, the generated forecast samples match the ground truth conditional probability distribution. Extensive tests using publicly available data from U.S. independent system operators under various point and probabilistic forecasting metrics demonstrate that WIAE-GPF consistently outperforms classical methods and cutting-edge machine learning techniques.

==> Simulation.tex <==
We conducted extensive experiments to compare leading GPF and point forecasting techniques based on a suite of performance metrics. This section summarizes our findings for three market applications where GPF is particularly valuable to system operators and market participants: (a)  LMP forecasting for the optimal bidding in NYISO's 5-minute real-time energy market,  (b) GPF for the interregional LMP spread for the Coordinated Transaction Scheduling (CTS) \cite{Pike&White:21} market between NYISO and PJM, and (c) ACE forecasting for regulation services using PJM's 15-second ACE data.  Common to these applications is that the forecasted variables are endogenously determined by the market operations. In contrast to exogenous variables such as wind/solar generations and inelastic demands, the LMP and ACE values are the results of dispatch and commitment optimization, where binding constraints introduce spikes in dual variables from which LMPs are computed. They are highly dynamic as shown in Fig.~\ref{fig:RTDA}.

\begin{figure}[htbp]
\vspace{-1em}
    \centering
    \includegraphics[width=0.7\linewidth]{figs/RTDA_Load.eps}
    \caption{Real-time, day-ahead LMPs, and load at Long Island, and real-time LMP at NYC July 2023.}
    \label{fig:RTDA}
    \vspace{-1.5em}
\end{figure}
\subsection{Baseline Methods in Comparison}
\begin{table*}[htbp]
    \centering
    \caption{\small{Comparison of the baselines.}}
    \vspace{0.5em}
    \begin{tabular}{|c|c|c|c|c|}
    \hline
        Algorithm&Forecasting Type &Time Series Model &Forecastor Output &ML Models \\
        \hline
        SNARX \cite{weron_forecasting_2008}  &Probabilistic &Semiparametric AR  &AR Model Parameters & Kernel Estimation\\
        \hline
        WIAE-GPF &Probabilistic &Nonparametric &Generative &CNN + WIAE\\
        \hline
        TLAE \cite{nguyen_temporal_2021} &Probabilistic &Parametric &Generative &RNN + VAE\\
        \hline              
        DeepVAR \cite{SalinasEtal:19NeuripsDeepVAR} &Probabilistic &Parametric (AR Model) &Model Parameters &LSTM\\
        \hline
        BWGVT \cite{BottieauEtal:23TPS}  &Probabilistic &Nonparametric &Forecasted Quantiles &LLM + Quantile Regression\\
        \hline
        Pyraformer \cite{liu_pyraformer_2022} &Point &Nonparametric  &Point Estimate &LLM\\
        \hline
        Informer \cite{ZhouEtal:21AAAI} &Point &Nonparametric  &Point Estimate &LLM\\
        \hline
    \end{tabular}
    \label{tab:comparison}
    % \vspace{-2em}
\end{table*}
We compared WIAE-GPF with six leading forecasters based on their relevance to power system applications and their established reputations. See Table \ref{tab:comparison} for attributes of these techniques and references. WIAE-GPF is the only nonparametric GPF forecaster. Because there are limited nonparametric GPF techniques, we also included in our comparison popular machine-learning-based parameterized GPF and point-forecasting techniques.

We started with SNARX \cite{weron_forecasting_2008}, a classical parametric forecasting technique based on an auto-regressive moving-average (ARMA) model. An early study showed that SNARX performed the best among a list of parametric techniques \cite{weron_forecasting_2008}.
For deep-learning techniques, we compared with DeepVAR \cite{SalinasEtal:19NeuripsDeepVAR}, a multivariate generalization of the popular DeepAR that has become a key baseline for time series forecasting in multiple applications.
Temporal Latent AutoEncoder (TLAE) \cite{nguyen_temporal_2021} is an autoencoder-based parametric GPF where the conditional distribution of the future time series variables is obtained through a transformed Gaussian random process with mean and variance as parameters.  Once these parameters are estimated from observed realizations, Gaussian Monte Carlo samples are fed into the decoder to generate samples of the forecasted random variable. 


We also included three popular forecasting techniques based on LLMs.  One is the award-winning technique Informer \cite{ZhouEtal:21AAAI}; the other is  Pyraformer \cite{liu_pyraformer_2022} that captures temporal dependency at multiple granularities\footnote{Pyraformer is the keynote presentation at The International Conference on Learning Representations (ICLR) 2022.}.  
Pyraformer showed superior performance over a wide range of LLM-based point forecasting techniques.
Specifically developed for LMP forecasting,  BWGVT\footnote{We have named the algorithm by the first letters of authors' last names}
\cite{BottieauEtal:23TPS} combines quantile regression with a transformer architecture derived for LLMs.  
% \vspace{-2em}
\subsection{Evaluation Metrics}  
Comparing probabilistic forecasting methods is difficult due to the lack of ground truth for the underlying conditional distribution. 
However, because a GPF can produce arbitrarily many Monte Carlo samples\footnote{We used $1000$ Monte-Carlo samples and sample average to obtain point estimates.}, it can be evaluated by all point forecasting metrics.
More importantly, an ideal probabilistic forecaster that produces the correct conditional distribution will perform well under any point estimator metric under regularity conditions. 
Therefore, evaluating a GPF method based on a set of point-forecasting techniques is a credible way to assess its performance.

We used four popular point forecasting and one widely used probabilistic forecasting metrics. 
See Appendix for their definitions. 
Normalized mean squared error (NMSE) measures the error associated with the mean of the estimated conditional probability distribution.  Normalized Absolute Error (NMAE) measures the error associated with the median. 
Mean absolute scaled error (MASE) is the ratio of the NMAE of a method over that of the (naive) persistent predictor that uses the latest observation available as the forecast. 
Symmetric mean absolute percentage error (sMAPE) averages and symmetrizes the percentage error computed at each time stamp and is less sensible to outliers. 
The probabilistic forecasting metric was the continuous ranked probability score (CRPS) \cite{TilmannEtal14ARStats}.
Additional simulations involving measures for quantile estimation can be found in \cite{WangTong24:arxiv}.

For probabilistic forecasting techniques, we used their conditional means as the point forecasts when evaluated by NMSE, whereas the conditional median is used for NMAE, MASE, and sMAPE. For the quantile regression technique, BWGVT, we use the estimated 0.5-quantile as its point forecast for all metrics since it's unclear how to compute empirical mean from quantiles.
\subsection{LMP forecasting for Energy Market Participation}
\label{subsec:RTDA}
\begin{table*}[htbp]
    \centering
    \caption{{\small Evaluation of forecasting results for real-time price forecasting at Long Island. The numbers in the parentheses were the ranking of the algorithm.  
The columns under the label of LONGIL are the GPF performance of the 12-step foresting of the LMP at LONGIL. The columns under LONGIL \& NYC are the performance of LMP forecasting at LONGIL using both LONGIL and NYC observations. }}
    \vspace{0.5em}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|}
    \hline
        \multirow{2}{*}{Methods} & \multicolumn{2}{c|}{NMSE}  & \multicolumn{2}{|c|}{NMAE}  &\multicolumn{2}{|c|}{MASE}  &\multicolumn{2}{|c|}{sMAPE} &\multicolumn{2}{|c|}{CRPS}
        % &\multicolumn{2}{|c|}{CRPS} 
        \\
        \cline{2-11}
          &LONGIL &LONGIL \& NYC  &LONGIL & LONGIL \& NYC  &LONGIL & LONGIL \& NYC &LONGIL & LONGIL \& NYC &LONGIL & LONGIL \& NYC
          \\
        \hline
        SNARX \cite{weron_forecasting_2008}  &$0.9852$ (7)  &$0.5029$ (7)  &$0.9733$ (7)  &$0.7318$ (7) &$0.7053$ (7)  &$0.4548$ (7) &$0.4319$  (7) &$0.4162$ (7)
          &$18.2864$ (3) &$10.5286$ (3)
         \\
         \hline
         WIAE-GPF  & $\mathbf{0.0585}$ (1)  &$0.0487$ (2)   &$\mathbf{0.2074}$ (1)   &$\mathbf{0.1186}$ (1) &$\mathbf{0.1503}$ (1) &$\mathbf{0.0737}$ (1) &$\mathbf{0.0839}$ (1)  &$\mathbf{0.0316}$ (1)
          &$\mathbf{4.0029}$ (1) &$\mathbf{1.1519}$ (1)
         \\
         \hline
         TLAE \cite{nguyen_temporal_2021}  &$0.2956$ (4)  &$\mathbf{0.0232}$ (1)  &$0.4186$ (6)  &$0.1366$ (2) &$0.3034$ (6) &$0.0849$ (2)  &$0.2720$ (3) &$0.3190$ (2)
          &$6.1875$ (2) &$2.8449$ (2)
         \\
         \hline
         DeepVAR \cite{SalinasEtal:19NeuripsDeepVAR} &{$0.3919$} (6) &{$0.4060$} (6) &{$0.4088$} (5) &{$0.4097$} (6) &{$0.2963$ (5)} &{$0.2546$} (6) &{$0.3629$} (5) &$0.3703$ (3)
          &$23.1460$ (4) &$22.9434$ (4)
         \\
         \hline
        BWGVT \cite{BottieauEtal:23TPS}  &$0.2670$ (3)  &$0.2528$ (5) &{$0.3158$} (4) &{$0.3280$} (5)
        &$0.2289$ (4) &$0.2038$ (5) &{$0.2817$} (4)&{$0.3900$} (6)&$24.2595$ (5) &$24.3065$ (5)\\
          \hline
         Pyraformer \cite{liu_pyraformer_2022}	&$0.3128$ (5)	&$0.1382$ (3)	&$0.3074$ (2) &$0.2556$ (3)	&$0.2228$ (2) &$0.1588$ (3)	&$0.1059$ (2) &$0.3765$ (4)
         &N/A &N/A
         \\
         \hline
         Informer \cite{ZhouEtal:21AAAI}    &$0.1912$ (2)   &$0.1829$ (4)  &$0.3147$ (3)   &$0.2830$ (4)  &$0.2281$ (3)   &$0.1759$ (4)    &$0.3761$ (6) &$0.3827$ (5) &N/A &N/A
         \\
         \hline
    \end{tabular}}
    \label{tab:RTDA-point}
    \vspace{-1.5em}
\end{table*}
\begin{figure*}
    \centering
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{figs/RTDA_WIAE.eps}
        \caption{WIAE-GPF}
    \end{subfigure}
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{figs/RTDA_Pyraformer.eps}
        \caption{Pyraformer}
    \end{subfigure}
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{figs/RTDA_SNARX.eps}
        \caption{SNARX}
        \label{fig:SNARX_RTDA}
    \end{subfigure}
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{figs/RTDA_DeepVAR.eps}
        \caption{DeepVAR}
    \end{subfigure}
    \caption{Trajectories of the real-time price at LONGIL, and its prediction generated by selective methods.}
    \label{fig:RTDA_traj}
\end{figure*}
% \begin{table*}[htbp]
%     \centering
%     \caption{Evaluation of probabilistic forecasting results of real-time prices at Long Island.}
%     \begin{tabular}{|c|c|c|c|c|c|c|}
%     \hline
%          \multirow{2}{*}{Methods} & \multicolumn{2}{|c|}{CRPS} & \multicolumn{2}{|c|}{Uncond. Cov. (90\%)} & \multicolumn{2}{|c|}{Uncond. Cov. (50\%)} \\
%          \cline{2-7}
%          &Long Island &Long Island \& NYC  &Long Island & Long Island \& NYC  &Long Island & Long Island \& NYC  \\
%          \hline
%          WIAE-GPF  &$\mathbf{4.6029}$ &$\mathbf{1.1519}$  &$\mathbf{0.9245}$ &$\mathbf{0.9157}$ &$\mathbf{0.5216}$ &$\mathbf{0.5184}$ \\
%          \hline
%          TLAE   &$6.1874$ &${2.8449}$  &\fbox{$0.9325$} &\fbox{$0.5920$}   &\fbox{$0.5423$} &\fbox{$0.3714$}\\
%          \hline
%          QuantGAM  &$29.7012$ &$28.7830$ &\fbox{$0.2050$} &\fbox{$0.1667$} &\fbox{$0.1273$} &\fbox{$0.0332$} \\
%          \hline
%          BWGVT  &$24.2595$ &$24.3065$ &{$0.9999$} &$0.9829$ &$0.9815$ &$0.9322$\\
%          \hline
%          SNARX  &$18.2864$ &$10.5286$  &\fbox{$0.6737$} &\fbox{$0.5221$} &\fbox{$0.2549$} &\fbox{$0.4254$} \\
%          \hline
%          Deep(V)AR &$23.1460$ &$22.9343$ &\fbox{$0.8425$}  &\fbox{$0.8408$ }&\fbox{$0.3363$ }&\fbox{$0.3512$} \\
%          \hline
%     \end{tabular}
%     \label{tab:RTDA_prob}
% \end{table*}
For a self-scheduled resource submitting a quantity bid to the energy market, the ability to forecast future prices is essential in constructing its bids and offers. 
With GPF generating future LMP realizations, the problem of optimal offer/bid strategies can be formulated as scenario-based stochastic optimization \cite{Tomasson&Hesamzadeh&Wolak:20AE}. 
Our experiment was based on a use case of a merchant storage owner submitting quantity offers and bids to a deregulated wholesale market, using LMP from NYISO as the hypothetical price realizations.

The real-time market of NYISO closes sixty minutes ahead of actual delivery, which means that the forecasting horizon needs to be longer than 60 minutes. 
Two experiments were conducted to produce probabilistic forecasts of 60-minute ahead LMPs at the Long Island (LONGIL) using (a) the day-ahead prices and the current and past real-time LMPs at LONGIL, along with the system load up to the time of submitting the bid; (b) the neighboring NYC real-time LMP in addition to the data in (a). 

Fig.~\ref{fig:RTDA} shows the real-time LMP trajectories at both LONGIL and NYC along with the demand and the day-ahead LMP at LONGIL.  
The real-time LMPs at LONGIL and NYC showed apparent spatial dependencies, while the dependency between day-ahead and real-time LMPs at LONGIL. 
The dependencies between load and real-time LMP were less obvious.
The real-time LMPs and load were collected every 5 minutes and day-ahead LMPs every hour.
We used the first 25 days for training and validation, and last 6 days of July for evaluation.

Test results are shown in Table \ref{tab:RTDA-point} with boldfaced numbers being the best performance.  
We observed that WIAE-GPF performed the best for all cases except for the forecasting of LONGIL LMP using both LONGIL and NYC data, for which WIAE-GPF is close second under NMSE. 
The strong performance of WIAE-GPF comes from that it aims to match conditional distribution, with a validity guarantee that ensures the Monte-Carlo samples generated have the same conditional distribution as that of the actual time series variable.
Overall, the second-best is TLAE; the VAE-trained RNN autoencoder achieved noticeable gain by combining data from two locations, especially for the joint forecasting at LONGIL \& NYC.
However, under the probabilistic forecasting measure of CRPS, TLAE was 50\% to 100\% higher than that of WIAE-GPF.  Because sampling the correlated Gaussian latent process is nontrivial, TLAE used a re-parameterization heuristic that could cause an accumulation of biases.  

The three LLM-based forecasters (BWGVT, Pyraformer, and Informer)  performed roughly the same, worse than WIAE-GPF and TLAE  but better than SNARX and DeepVAR. Note that Pyraformer and Informer are both point forecasters trained to minimize the mean squared forecasting error.  They did not perform well under NMAE, MASE, and sMAPE.
BWGVT is adapted to be a probabilistic forecaster, although it did not perform well under the CRPS score. 
Its quantile prediction was outlier-sensitive, especially when compared with the GPF methods that depend on the stochastic latent process.
Hence, both their point estimation results and CRPS were worse than TLAE and WIAE-GPF.

For the two parametric techniques, the parametric DeepVAR, being significantly simpler than LLM forecasters, performed slightly worse.  The pre-deep-learning era SNARX performed the worst across the board. The inaccurate semiparametric-AR model assumption appears to be culpable.
Their performance was influenced by model mismatch, where ARMA models typically expect smoother trajectories.
For the real-time LMP that exhibits high volatility, these methods are slow to catch the rapid change, leading to predicting shifted peaks that resulted in huge forecasting errors, which is corroborated by their high sMAPE that indicates a higher percentage error at each time stamp.

It is interesting to observe that using LMPs in neighboring locations improved the forecasting performance of all methods except DeepVAR and BWGVT, as shown by the LONGIL and LONGIL \& NYC columns under the DeepVAR and BWGVT rows in Table~\ref{tab:RTDA-point}.
This implies that these two methods didn't account for spatial correlations optimally.
We conclude this to the difficulty of training of transformer and LSTM models.

To gain insights into the performance of WIAE-GPF and other benchmark techniques, we plotted the ground truth trajectories (black) and trajectory forecasts generated by WIAE-GPF (red) and a competing algorithm (blue) in Fig.~\ref{fig:RTDA_traj}.
Note that the spikes were not predicted by any methods.  
This was not surprising given the nature of how these spikes were produced.  Aside from these spikes, these figures show clearly that WIAE-GPF (red) tracked the ground truth (black) the closest, which was supported by the fact that WIAE-GPF has the smallest NMAE.  We also observed that WIAE-GPF had the smallest variation, which is supported by the fact that WIAE-GPF had the smallest NMSE. 
Furthermore, WIAE-GPF was the least affected by the price spikes. 
This was because, as a GPF method, the Monte-Carlo samples used to produce the MMSE point estimate were less likely to include extreme samples.  However, for SNARX, as shown in Fig.~\ref{fig:SNARX_RTDA}, the spikes caused significant deviations from the forecasted trajectory. 
% \vspace{-1em}
\subsection{Forecasting for Interchange Markets}
\label{subsec:spread}
The interchange market aims to improve overall economic efficiency across ISOs by allowing virtual bidders to arbitrage price differences at proxy buses of two neighboring ISOs.  This experiment was based on the use case of a virtual bidder bidding into the CTS market between NYISO and PJM. The proxy buses of this market were Sandy Point of NYISO and Neptune of PJM.

The CTS market closes 75 minutes ahead of delivery and is cleared every 15 minutes. A virtual bidder submits a price-quantity bid along with the direction of the virtual trade from the source of the proxy with low LMP to the destination proxy with high LMP.  Once the market is cleared, the settlement is based on the actual LMP spread between the two proxies and the cleared quantity.   
The bidder profits if the virtual trade direction matches the direction of the real-time LMP spread. 
Otherwise, the bidder incurs a loss. 
Therefore, the ability to predict the LMP spread direction is especially important.

We performed a 75-minute ahead LMP spread forecasting using the interface power flow and LMP spread data between NYISO and PJM at the Neptune proxy, collected in February 2024.
The interface power flow samples were collected every 5 minutes, and LMP spread every 15 minutes.
We used the first 24 days for training and validation, and the last 5 days of February for testing.


We added {\em Prediction Error Rate (PER)} as a measure for the accuracy of the virtual trading direction prediction, given that the sign of spread is of great importance to profitability. 
PER indicates the percentage of forecasts that don't have the same direction as the ground truth.
For point forecasts, we compared the signs of the forecasts with the signs of the ground truth. 
For probabilistic forecasting, we compared the direction of the ground truth with that of the minimum error-probability prediction of the LMP spread, which is the sign of the conditional median.
For GPF, we compare the sample median with the sign of the ground truth.

\begin{table}[htbp]
    \centering
    \caption{{\small Evaluation of forecasting results for spread forecasting between NYISO and PJM.}}
    \vspace{0.5em}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{|c|c|c|c|c|c|c|}
    \hline
        {Methods} & {NMSE}  & {NMAE}  &{MASE}  &{sMAPE} &PER  &CRPS
        % &\multicolumn{2}{|c|}{CRPS} 
        \\
        \hline
        SNARX \cite{weron_forecasting_2008} &{$2.4531$} (7)   &{$1.3415$} (7)   &$1.1847$ (7)  &{$0.4958$} (7)&$0.6781$ (7) &$120.0403$ (5)
         % &$11.3431$ &$28.8337$
         \\
         \hline
         WIAE-GPF  & $\mathbf{0.0098}$ (1)     &$\mathbf{0.2738}$ (1)    &$\mathbf{0.2418}$ (1)  &$\mathbf{0.4493}$ (1) &$\mathbf{0.0606}$ (1) &$\mathbf{4.0329}$ (1) 
         % &$\mathbf{0.8238}$ 
         % &$\mathbf{0.4156}$  
         \\
         \hline
         TLAE \cite{nguyen_temporal_2021}  &$0.9592$ (5)  & $0.9785$ (5)  &$0.8641$ (5)  &$0.4785$ (4)&$0.3692$ (4)&$15.5195$ (2) 
         % &$2.8167$ &$3.1743$
         \\
         \hline
         DeepVAR \cite{SalinasEtal:19NeuripsDeepVAR}  &{$1.8986$} (6)  &$0.7224$ (3)  &{$0.6380$} (3)  &{$0.4806$} (5)&$0.3505$ (3)&$32.8296$ (4)
         % &$2.1392$ &$2.7981$ &$$
         \\
         \hline
         BWGVT \cite{BottieauEtal:23TPS}  &{$0.9053$} (3)&{$0.8525$} (4) &{$0.7529$} (4) &{$0.4674$} (3)&$0.2313$ (2)  &$31.5660$ (3)\\
         \hline
         Pyraformer \cite{liu_pyraformer_2022} 	&$0.9478$ (4)		&{$1.2674$} (6) 	&{$1.1193$} (6) 	&{$0.4909$} (6)&$0.6738$ (6)&N/A
         % &N/A &N/A
         \\
         \hline
         Informer \cite{ZhouEtal:21AAAI}      &$0.8045$ (2)      &$0.4185$ (2)       &$0.4252$ (2)        &$0.4580$ (2) &$0.5487$(5) &N/A
         \\
         \hline
    \end{tabular}}
    \label{tab:spread}
\end{table}
% \begin{table}[htbp]
%     \centering
%     \caption{Probabilistic forecasting results of spread forecasting between NYISO and PJM.}
%     \begin{tabular}{|c|c|c|c|}
%     \hline
%          Methods & CRPS & {Uncond. Cov. (90\%)} & {Uncond. Cov. (50\%)}  \\
%          \hline
%          WIAE-GPF  &$\mathbf{4.0329}$  &$\mathbf{0.9215}$  &${0.4726}$\\
%          \hline
%          TLAE  &$15.5195$  &$0.8557$  &$\mathbf{0.5052}$\\
%         \hline
%          BWGVT  &{$31.5660$}  &{$0.9989$}  &$0.6835$ \\
%          \hline
%          SNARX  &$120.0403$   &{$0.3557$}  &$0.2042$\\
%          \hline
%          DeepAR &{$32.8296$} &$0.3355$  &${0.1480}$\\
%          \hline
%     \end{tabular}
%     \label{tab:spread_prob}
% \end{table}

{
Seen from Table \ref{tab:spread}, WIAE-GPF performed better than all other techniques in all metrics.
TLAE performed the second-best in CRPS ($15.5195$) but slightly worse than BWGVT when evaluated under point estimation metrics.
Its sequential sampling of the latent Gaussian process added to its numerical instability.
BWGVT was the overall second-best performing probabilistic technique.
Its transformer architecture with enhanced capability of capturing long-term temporal dependency didn't offer so much gain as to the training difficulty imposed by the increasing number of deep-learning parameters, see \cite{WangTong24:arxiv}.
Point estimation techniques, namely Pyraformer and Informer, were not competitive when evaluated under point estimation metrics other than NMSE.
Among probabilistic methods, DeepVAR performed similarly to the LLM methods, and SNARX had the most difficulties.
These (semi) parametric methods suffered from model mismatch, and were sensitive to sudden changes,
Thus, shifted peaks and valleys were often witnessed in their predictions.
} 
% \vspace{-1em}
\subsection{ACE Forecasting for Reserve Market Participants}
ACE is defined as the difference between actual and scheduled load-generation imbalance, adjusted by the area frequency deviation \cite{NERC:11}.  It is the control signal for frequency regulation, and its probabilistic forecasting is especially important for the operator to procure resources and market participants to bid in the regulation ancillary service market.

{
In this subsection, we present the simulation results of a 5-minute ahead forecasting of ACE.
We utilized the ACE data from Jan 24th to 26th, collected by PJM.
The ACE signal is measured every 15 seconds and can be quite volatile.}
% \begin{figure}[htbp]
%     \centering
%     \vspace{-1em}
%     \includegraphics[width=0.8\linewidth]{figs/ACE.eps}
%     \caption{Trajectory of ACE at PJM, Jan. 24th - 26th, 2023.}
%     \label{fig:ACE}
% \end{figure}
\begin{table}[htbp]
    \centering
    \caption{{\small Estimation Results of ACE forecasting for PJM. The prediction step is 5-minute ahead.}}
    \vspace{0.5em}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{|c|c|c|c|c|c|}
    \hline
         Methods    &NMSE   &NMAE   &MASE   &sMAPE &CRPS \\
         \hline
         SNARX \cite{weron_forecasting_2008}  &$1.1922$ (6)&$1.1303$ (6)&$0.7029$ (6)&$0.4605$ (6)&$2.1007$ (5)\\
         \hline
         WIAE-GPF     &$\mathbf{0.5957}$ (1)&$\mathbf{0.7555}$ (1)&$\mathbf{0.4698}$ (1)&$\mathbf{0.1059}$ (1)&$\mathbf{0.0081}$ (1)\\
         \hline
         TLAE \cite{nguyen_temporal_2021}      &$1.1727$ (5)&$1.0605$ (5)&$0.6595$ (5)&$0.2782$ (3)&$1.5541$ (4)\\
         \hline
         DeepVAR \cite{SalinasEtal:19NeuripsDeepVAR} &$1.4431$ (7)&$1.1750$ (7)&$0.7307$ (7)&$0.3952$ (5)&$1.2947$ (3)\\
         \hline
         BWGVT \cite{BottieauEtal:23TPS} &$0.9562$ (3)&$0.9793$ (2)&$0.6090$ (2)&$0.3168$ (4)&$1.2488$ (2)\\
         \hline
         Pyraformer \cite{liu_pyraformer_2022} &$0.9783$ (4)&$0.9948$ (4)&$0.6186$ (4)&$0.4986$ (7)&N/A\\
         \hline
         Informer \cite{ZhouEtal:21AAAI} &$0.6006$ (2)&$0.9819$ (3)&$0.6106$ (3)&$0.2247$ (2)&N/A\\
         \hline
    \end{tabular}}
    \label{tab:ACE_20_point}
\end{table}
% \begin{table}[htbp]
%     \centering
%     \caption{Probabilistic Estimation Results of ACE forecasting for PJM. The prediction step is 5-minute ahead.}
%     \begin{tabular}{|c|c|c|c|}
%     \hline
%         Methods & CRPS &Uncond. Cov.(90\%) &Uncond. Cov.(50\%)  \\
%         \hline
%          WIAE-GPF &$\mathbf{1.0081}$  &$\mathbf{0.8984}$  &$\mathbf{0.5321}$\\
%          \hline
%          TLAE &$1.5541$ &$0.1143$ &$0.0511$\\
%          \hline
%          BWGVT &$1.2488$ &$0.9065$ &$0.5754$\\
%          \hline
%          SNARX &$2.1007$ &$0.0740$ &$0.0203$\\
%          \hline
%          DeepAR &$1.2947$ &$0.5474$ &$0.2440$\\
%          \hline
%     \end{tabular}
%     \label{tab:ACE_20_prob}
% \end{table} 
WIAE-GPF achieved better performance than other methods, with CRPS less than $0.01$ and sMAPE less than $11\%$, as shown by the WIAE-GPF row.
We credited the strong performance of WIAE-GPF to the simplicity of its latent process, and its Bayesian sufficiency.
BWGVT ranked second among all methods since the ACE data has few outliers.
But its CRPS at $1.2488$ is dramatically larger than that of WIAE-GPF.
Pyraformer and Informer, trained with NMSE, had better performance under NMSE but worse under NMAE.
With NMSE over $110\%$, TLAE had the worst performance among GPF methods.
DeepVAR and SNARX performed worse than the other forecasting methods, with NMSE and NMAE larger than $110\%$, possibly due to model mismatch.
% \vspace{-1em}
% \subsection{Discussion: On using LLM}
% \label{subsec:discussion}
% As LLM forecasters techniques, Pyraformer, Informer and BWGVT performed better than the more conventional SNARX (see {Table~\ref{tab:RTDA-point}, \ref{tab:spread}, \ref{tab:ACE_20_point}}). Compared with the more straightforward deep learning method of DeepVAR, LLM-based forecasting did not show clear advantages. The same can be said when they were compared with TLAE.

% To understand if long-range dependencies matter in the probabilistic forecasting of electricity market signals, we examined the characteristics of LMP signals using the Hurst exponent and Detrended Fluctuation Analysis (DFA) as indicators for the long-range dependencies of LMP; both parameters had the range [0,1], with deviation from 0.5 indicating symptoms of long-range dependencies.

% \begin{table}[htbp]
%     \centering
%     \vspace{-1em}
%     \caption{{\small Statistics that models long-range dependency of time series.}}
%     \vspace{0.5em}
%     \begin{tabular}{|c|c|c|c|}
%     \hline
%          Metrics &Real Time &Interchange Spread & ACE\\
%     \hline
%         Hurst Exponent  &$0.5257$ &$0.5301$ &$0.5351$\\
%     \hline
%         DFA &$0.6053$ &$0.6614$ &$0.8609$\\
%     \hline
%     \end{tabular}
%     \label{tab:LR}
% \end{table}

% Table~\ref{tab:LR} shows the estimated Hurst exponent and DFA.   The Hurst Exponent and DFA slope displayed a slight deviation from 0.5. The English and Korean literature \cite{MontemurroPury:02Fractals,BhanEtal:06CSF} are known to have long-range dependencies with the Hurst exponents ranging from 0.64 to 0.73. In comparison, the long-term effect of real-time electricity market signals is minimal.
% The fact suggests that the use of LLM may not be suitable for electricity market signals where long-range dependencies are not evident. Indeed, real-time LMPs are computed either on an interval-by-interval basis or as part of short sliding window economic dispatch. Any temporal coupling is a result of temporal dependencies of demand and supplies, neither shown to have long-range dependencies. An unproven hypothesis is that the model complexity of LLM may offset any benefit it may bring to price forecasting.
% \subsection{Discussion}

% Table~\ref{tab:LR} exhibits the estimators that model the long-range dependency of a time series.
% We computed the Hurst exponent and Detrended Fluctuation Analysis (DFA) estimator.
% These two metrics range from $0$ to $1$, with the deviation from $0.5$ indicating the persistence of long-range dependency, \ie, Hurst exponent equals to $0.5$ indicates that the time series is temporally independent.
% Hurst exponent represents the probability that the direction (up or down compared to the previous value) of the next value is more likely to be the same as the direction of the current value.
% DFA computes the difference (size of fluctuation $F(n)$) between the observations and a lease-square regression using an interval of $n$ samples.
% Then the slope of the double logarithmic plot of $F(n)$ as a function of $n$ is computed as an indication of long-range dependency.
% For a detailed definition of Hurst Exponent and DFA, see \cite{StroeEtaL:09BRM}.
% Seen from Table~\ref{tab:LR}, the Hurst Exponent and DFA slope displayed a slight deviation from $0.5$.
% Compared with the Hurst exponents of English and Korean literature \cite{MontemurroPury:02Fractals,BhanEtal:06CSF}, which typically range from $0.64$ to $0.73$, the long-term effect of real-time electricity market signals is minimal, with their Hurst exponent below $0.6$.
% These metrics corroborated that temporal dependency doesn't persist in electricity price data series, and hence adopting complicated deep learning architecture employed by Pyraformer, Informer, and BWGVT doesn't offer much gain in forecasting performance.
% Previous observations showed that naive forecasters can be hard to beat for real-time market variables~\cite{KlaeboeEtal:15ES}.

% The ARMA-based parametric techniques suffer from model mismatch.
% Furthermore, the fact that their estimated parameters are heavily affected by past observations of $(\Xbf_t)$ makes them unsuitable for predicting spiky trajectories of real-time market signals.
% When historical data contains spikes with large magnitudes, DeepAR, QuantGAM, and SNARX exhibited the phenomenon of predicting shifted peaks and valleys, adding to both point and probabilistic forecasting errors.

% Nonparametric GPF, leveraging latent process to generate future samples from conditional distributions, achieved overall better performance.
% TLAE learns a correlated Gaussian process and its latent process, while WIAE-GPF learns IID uniform innovation representation.
% Due to the complicated probability structure of its latent process, TLAE demands a sequential sampling of latent samples based on the realization of the previously sampled latent variable.
% When the prediction step increases, the sequential sampling process accumulates bias and statistical instability, affecting the quality of future samples acquired.
% On the other hand, the sampling of innovation representation is simple and computationally efficient, contributing to WIAE-GPF's success in real-time market forecasting tasks.


==> formulation.tex <==
We consider a GPF problem of energy system-related time series.
Let $(\Xbf_t)$ denote the $d$-dimensional random process\footnote{for a $d$-dimensional random process, $\Xbf_t=(X_t^1,X_t^2,\cdots,X_t^d)$, $\forall t$} whose historical realizations is publicly available.
At each time stamp $t$, the random vector $\Xbf_t$ consists of $d$ univariate random processes of same sampling frequency, which represent different quantities.
Depending on requirements of any specific application, market participants are only interested in forecasting the probabilistic distribution of a nonempty subset (denoted by $\Dc_f$) of time series in $\Xbf_t$ at future time stamps.
We denote the cardinality of $|\Dc_f|$ by $d_f$.
The subset of time series that we wish to predict is named in similar fashion as $(\Xbf^f_t)$, where $\Xbf^f_t=(X_t^{i_1},X_t^{i_2},\cdots,X_t^{i_{d_f}}),\forall t$, where $\Dc_f = \{i_1,i_2,\cdots,i_{d_f}\}$. 
In our formulation, $\Xbf_t^f$ should contain the subset of time series that are directly related to decision-making, such as spread for virtual trader, and real-time electricity price for energy storage participator.

While probabilistic forecasting techniques aim to estimate the conditional distribution of $\Xbf^f_t$ given past observations of $\Xbf_t$, GPF techniques, being generative at core, aim to produce Monte Carlo samples distributed according to the same conditional distribution.


% When $d_f<d$, at least one time series is used solely as the covariate of forecasting, whose future distributions is not of interest.
% We denote those time series as $\Xbf_t^c$, with the superscript $c$.
% In real-world applications, $\Xbf_t^c$ may include temperature and load data, which are not of primary interest to virtual traders.
% In nutshell, the time series forecasting problem we are considering involves utilizing historical observations of $\Xbf_t$ to predict the conditional distribution of $\Xbf_t^f$ at future timestamps.

In the rest of the paper, time series viewed as random processes will be denoted by boldface capitalized letters (e.g., $\Xbf_t$ and $\Vbf_t$), with their subscript being time indices.
The realizations of each time series are denoted by the corresponding boldface lowercase letters (e.g., $\xbf_t$ and $\vbf_t$).
Without further explanation, we will use $t$ to reference the present time stamp.
To further simplify the notations with respect to reference time, the set of realized random vectors of any given time series is denoted by its script type font, e.g., $\Xmsc_t :=\{\Xbf_t, \Xbf_{t-1},\cdots\}$ and $\Vmsc_t :=\{\Vbf_t, \Vbf_{t-1},\cdots\}$.
Similarly, we use $\mathbf{x}_t:=\{\xbf_t,\xbf_{t-1},\cdots\}$ to denote the set of past observations.
Hence, $\Xmsc_t = \mathbf{x}_t$ indicates the event where the random vectors in the past equals to their realized values, i.e., $\{\Xbf_t = \xbf_t,\Xbf_{t-1} = \xbf_{t-1},\cdots\}$.

==> training.tex <==
For most real-world scenarios, the probability distribution of $(\Xbf_t)$ is hard to characterize, and thus the WIAE functions $(G,H)$ are generally unknown.
This demands a learning algorithm to obtain $(G,H)$ from historical data.
In this section, we recount the deep-learning architecture and its training objective, that are proposed to approximate WIAE $(G,H)$ in a data-driven way.

Shown in Fig.~\ref{fig:schematic} is the schematic that highlights key components of the WIAE learning.
The encoder $G_\theta$ and decoder $H_\eta$ are causal convolutional neural networks \cite{Waibel&etal:89} parameterized by neural network coefficients $\theta$ and $\eta$, respectively.  
The neural network-parameterized weak innovation encoder $G_\theta$ takes time-shifted segmentation of $(\Xbf_t)$ as input, the length of which is denoted by $m$.
This means that a single input to $G_\theta$ consists of $m$ consecutively sampled historical observations of $(\Xbf_t)$, i.e., $(\Xbf_t,\Xbf_{t-1},\cdots,\Xbf_{t-m+1})$.
The output of $G_\theta$ is a single estimate of the weak innovation sequence at time $t$, which we denote by $\hat{\Vbf}_t$.
Similarly, the input to the neural network parameterized decoder $H_\eta$ is also a $m$-dimensional segmentation of $(\hat{\Vbf}_t)$.
To this end, $m$ represents the "filter memory" of the autoencoder pair.

The two deep-learning components, $(G_\theta,H_\eta)$, serve as a $m$-dimensional data-driven approximation to the WIAE transformation pair $(G,H)$.
Their neural network parameters are learned by optimizing a specifically designed learning objective, to ensure that $(\hat{\Vbf}_t)$ is an accurate estimation of $(\Vbf_t)$.
The details of the training algorithm to obtain the optimal weights are described in Sec.~\ref{subsec:training}.

One should question that to what extent does $(\hat{\Vbf}_t)$ approximate $(\Vbf_t)$, if the WIAE function pair $(G,H)$ is infinite dimensional.
With $G$ and $H$ being infinite dimensional, existing data-driven implementation of $(G,H)$ can never achieve perfect approximation, no matter what training objective is applied. 
To address this concern, we present a structural convergence result which accounts for the asymptotic behavior of $(\hat{\Vbf}_t)$ as the dimensionality of filter memory $m$ grows to infinity.
The discussion can be found in Sec.~\ref{subsec:structural_conv}.
\subsection{Training of WIAE}
\label{subsec:training}
Weak innovation representation, at its core, are the matching of input-output distribution and the independence and identicality of the latent process $(\Vbf_t)$.
Hence, the training criterion of WIAE should reflect these two points depicted by Eq.~\eqref{Eq:iid}~\&~\eqref{Eq:recons} to arrive at the optimal parameters.
In this paper, we introduce two additional neural network structures, namely innovations discriminator $D_\gamma$ and reconstruction discriminator $D_\omega$, to enforce that these two equality.
The subscripts denote their corresponding neural network parameters.

The training schematics is outlined by Fig.~\ref{fig:schematic}.
\begin{figure}[htbp]
    \centering
    \includegraphics[width=\linewidth]{figs/Mul_IAE_training.eps}
    \caption{Training schematices of GPF-WI.}
    \label{fig:schematic}
\end{figure}
The two discriminators discriminate between distributions.
In particular, the {innovations discriminator $D_\gamma$} facilitate the comparison between the distributions of $(\Vbf_t)$ and an i.i.d. sequence of $d-$dimensional uniform random vector $\Ubf_t$, and the {reconstruction discriminator $D_\omega$} the comparison between the distributions of $(\Xbf^f_t)$ and $(\hat{\Xbf}^f_t)$. 

Here, we use the two discriminators to measure the Wasserstein distance $W(\cdot,\cdot)$ between distributions.
Wasserstein distance, metricizing weak convergence, can be computed by the famous Kantorovich-Rubinstein duality \cite{Villani09:Book} (Theorem 5.10).
This duality shows that the Wasserstein distance bewteen two random variables $X\sim f_1$ and $Y\sim f_2$ is equal to the maximum expected difference between $D(X)$ and $D(Y)$ under a 1-Lipschitz function $D$:
\begin{align}
    W(f_1,f_2) = \max_{D:\mbox{\small 1-Lipschitz}}\left(\mbbE_{X\sim f_1}[D(X)]-\mbbE_{Y\sim f_2}[{D}(Y)]\right).
    \label{eq:wass}
\end{align}
In \cite{Arjovsky17}, the authors proposed a Wasserstein GAN that employs a $\omega$-parameterized neural network for the 1-Lipschitz discriminating function $D_\omega$, where $\omega$ is optimized through \eqref{eq:wass}.
Adopting the same paradigm, we train deep neural network discriminators $D_\gamma$ and $D_\omega$ according to the duality in \ref{eq:wass} to estimate Wasserstein distances between the distributions of two random variables.

Tailoring to WIAE training, the two discriminator networks $D_\gamma$ and $D_\omega$ provide means to compute Wasserstein distances between $(\Vbf_t)$ and $(\Ubf_t)$, and between $(\Xbf_t)$ and $(\hat{\Xbf}_t)$.
The training objective of WIAE can thus be constructed as a weighted combination between two Wasserstein distances:
\begin{multline}
     L((\Xbf_t),\theta,\eta):= \max_{\gamma,\omega}\big(\mbbE[D_{\gamma}(\Ubf_t) - \mbbE[D_\gamma(\Vbf_{t})]] \\
     + \lambda(\mbbE[D_{\omega}(\Xbf^f_{t})]
      -\mbbE[D_{\omega}(\hat{\Xbf}^f_{t})])\big),
  \label{eq:loss}
\end{multline}
where $\lambda$ is a real number that scales the two Wasserstein distances.
Since the two parts of loss function \eqref{eq:loss} regularize $(G_\theta,H_\eta)$ according to \eqref{Eq:iid} and \eqref{Eq:recons}, minimizing the loss with respect to $\theta$ and $\eta$ is thus equivalent to enforcing $(\Vbf_t)$ being i.i.d uniform, and $(\hat{\Xbf}^f_t)$ having the same distribution as $(\Xbf^f_t)$. 

Though we would like to compute the Wasserstein distance between two infinite time series, this is impractical in nature, due to finite implementation of deep-learning architecture.
The discriminators can only discriminate finite segments of time series.
We denote the dimensionality of the input segmentation to discriminators by $n$.
For instance, the input segments to the innovation discriminator $D_\gamma$ are $(\hat{\Vbf}_t,\hat{\Vbf}_{t-1},\cdots,\hat{\Vbf}_{t-n+1} )$ and $(\Ubf_t,\Ubf_{t-1},\cdots,\Ubf_{t-n+1})$.

A keen observation to the finite implementation is that it cannot ensure the estimation of weak innovations $(\hat{\Vbf}_t)$ being an i.i.d. sequence, nor ensure that $(\hat{\Xbf}_t)$, as an infinite time series, has the same probability structure as $\Xbf_t$, even if the loss function in \eqref{eq:loss} is minimized to $0$.
This is a result of discriminators' limitation of failing to compare the Wasserstein distance between two random processes.
We argue that such a compromise is suboptimal yet inevitable, unless a practical way of constructing infinite dimensional deep-learning networks.
The effect of this compromise will be discussed in the following section.

\subsection{Structural Convergence of WIAE}
\label{subsec:structural_conv}
This section focuses on the practical issue raised by the finite implementation of neural network-parameterized WIAE and discriminators.
It is evident that with finite implementation, no learning objective and deep-learning architecture can guarantee a perfect approximation of WIAE transformation pair $(G,H)$, even if the amount of historical samples available is infinite.
Therefore, a way of qualitatively characterizing the asymptotic behavior of the estimation $(G_\theta,H_\eta)$ to the true function pair $(G,H)$ becomes essential.

We first introduce the notations used in this section, highlighting the finite dimensionality of the deep neural networks involved. 
For an $m$-dimensional WIAE, we denote encoder and decoder output sequence by $(\hat{\Vbf}_{m,t})$ and $\hat{\Xbf}_{m,t}$, with the additional subscript $m$.
% Likewise, the inputs to an $n$-dimensional innovation discriminator $D_{\gamma_n}$ is $\Vbf_t^{(n)} = (V_{m,t},\cdots, V_{m,t-n+1}$ and $\Ubf_t^{(n)}=(U_t,\cdots U_{t-n+1})$, and the inputs for the reconstruction discriminator are similarly defined $\Xbf_t^{(n)}$ and $\hat{\Xbf}^(n)_t$. 
Let the superscript $*$ denote the optimal parameters obtained via minimizing Eq.~\eqref{eq:loss}, i.e., $\theta_m^*$ and$\eta_m^*$.
Likewise, we denote the corresponding sequences computed by WIAE with optimal parameters by $(V_{m,t}^*)$, $(X_{m,t}^*)$. 
For simplicity and conciseness, we use the superscript $(n)$ with to indicate a $n$-dimensional finite vector, e.g., $\Vbf_{m,t}^{(n)}:=(\Vbf_{m,t},\Vbf_{m,t-1},\cdots,\Vbf_{m,t-n+1})$.
The same superscript combined with the loss function $L((\Xbf_t),\theta,\eta)$ indicate that the loss function is computed by $n$-dimensional discriminators.

To analyze the asymptotic property of WIAE approximation, we make the following assumptions:
\ben
\item[A1] {\bf Existence:}  The random process $(\Xbf_t)$  has a weak innovations representation defined in (\ref{Eq:encoder} - \ref{Eq:decoder}), and there exists a causal WIAE function pair $(G, H)$ with $H$ continuous.
\item[A2] {\bf Feasibility:} There exists a sequence of finite-dimensional auto-encoder functions $(G_{\tilde{\theta}_m}, H_{\tilde{\eta}_m})$ that converges uniformly to $(G,H)$ as $m\rightarrow \infty.$
\item[A3] {\bf Training:} The training sample sizes are  infinite. The training algorithm for all finite dimensional WIAE using finite dimensional training samples converges almost surely to the global optimum.
\een
\begin{definition}[Convergence of finite block $n$]
For all fixed $n\in\mathbb{Z}^+$, an $m$-dimensional WIAE trained with $n$-dimensional discriminators converges in distribution of finite block $n$ to the weak innovations sequence $(V_t)$ if, for all $t$,
\begin{align}
    (\hat{\Vbf}^{*}_{m,t},\cdots,\hat{\Vbf}^*_{m,t-n+1}) \stackrel{d}{\rightarrow} (\Vbf_t,\cdots,\Vbf_{t-n+1}), \\
    (\hat{\Xbf}^{*}_{m,t},\cdots,\hat{\Xbf}^*_{m,t-n+1}) \stackrel{d}{\rightarrow} (\Xbf_t,\cdots,\Xbf_{t-n+1}),
\end{align}
as $m\rightarrow\infty$.
\label{def:convergence}
\end{definition}
\begin{theorem} 
\label{thm:converge}
Under (A1-A3),  $(V_{m,t})$ converges (of finite block size $n$) to $(V_t)$, $\forall n \in \mathbb{Z}+.$
\end{theorem}
% {\em Proof:}
% Denote the $n$-dimensional vector $[V_{t,m}^{*(n)},\cdots,V_{t-n+1,m}^{*(n)}]$ by $\boldsymbol{V}_{t,m}^{*(n)}$, with the letter changed to bold face.
% ${\boldsymbol U}_{t,m},\hat{\boldsymbol X}_{t,m}^{(n)}$ and $\boldsymbol X^{(n)}_{t,m}$ are defined similarly. $\{\tilde{V}_t\}$ is the sequence generated by $G_{\tilde{\theta}_m}$. All the random variables generated by $(\tilde{\theta}_m,\tilde{\eta}_m)$ are defined in the similar pattern.
{\em Proof:} 
\ben
\item Want to show that
$L^{(n)}((\Xbf_t),\theta_m^*,\eta_m^*)\rightarrow 0$ as $m\rightarrow \infty$.

By assumption A2, $G_{\tilde{\theta}_m}\rightarrow G$ uniformly. 
Therefore, $\forall \epsilon$, there exists a $M$ such that  $\lVert \tilde{ \Vbf}_{t,m}^{(n)}- \Vbf_t^{(n)}\rVert<n\epsilon$ for $\forall m>M$. 
Thus $\tilde{ \Vbf}_{t,m}^{(n)}\stackrel{d}{\Rightarrow}\Vbf_t^{(n)}$. 
Similarly, we have 
\begin{multline*}
\big(H_{\tilde{\eta}_m}(\Vbf_{t},\cdots,\Vbf_{t-m+1}),\cdots,\\H_{\tilde{\eta}_m}(\Vbf_{t-n+1},\cdots,
\Vbf_{t-n-m+2})\big)\stackrel{d}{\Rightarrow} (\Xbf_t,\cdots,\Xbf_{t-n+1}).
\end{multline*}

Since $H$ is continuous and $H_{\tilde{\eta}_m}$ converge uniformly to $H$, $H_{\tilde{\eta}_m}$ is also continuous. Thus by continuous mapping theorem, $H_{\tilde{\eta}_m}(\tilde{\Vbf}_{t,m},\cdots,\tilde{\Vbf}_{t-m+1,m})\stackrel{d}{\Rightarrow}H_{\tilde{\eta}_m}(\Vbf_{t},\cdots,\Vbf_{t-m+1})$. 
Therefore, 
\[\tilde{\hat{\Xbf}}_{m,t}^{(n)}\stackrel{d}{\Rightarrow} \tilde{\Xbf}_{t}^{(n)}, L^{(n)}((\Xbf_t),\tilde{\theta}_m,\tilde{\eta}_m)\rightarrow 0.\]

Since $\theta^*$ and $\eta^*$ are the optimal parameters obtained by minimizing \eqref{eq:loss},
\begin{multline*}
L^{(n)}((\Xbf_t),\theta_m^*,\eta_m^*):=\min_{\theta,\eta}L^{(n)}((\Xbf_t),\theta,\eta)\\ \leq L^{(n)}((\Xbf_t),\tilde{\theta}_m,\tilde{\eta}_m)\rightarrow 0.
\end{multline*}

\item Since $L((\Xbf_t),\theta_m^*,\eta_m^*)\rightarrow 0$ as $m\rightarrow \infty$, by Eq.~\eqref{eq:loss}, $\boldsymbol V_{t,m}^{(n)} \stackrel{d}{\Rightarrow} \boldsymbol U_{t,m}^{(n)}$, $\hat{\boldsymbol X}_{t,m}^{(n)}\stackrel{d}{\Rightarrow}\boldsymbol X^{(n)}_{t,m}$ follow directly by the equivalence of convergence in Wasserstein distance and convergence in distribution \cite{Villani09:Book}.
\een
